Could the classical relativistic electron be a strange attractor?

We review the formulation of the problem of the electromagnetic self-interaction of a relativistic charged particle in the framework of the manifestly covariant classical mechanics of Stueckelberg, Horwitz and Piron. The gauge fields of this theory, in general, cause the mass of the particle to change. We show that the non-linear Lorentz force equation for the self-interaction resulting from the expansion of the Green's function has chaotic solutions. We study the autonomous equation for the off-shell particle mass here, for which the effective charged particle mass achieves a macroscopic average value determined by what appears to be a strange attractor.

==> ddcaptions.tex <==
\magnification=\magstep1
\bigskip
\bigskip
\centerline{\bf CAPTIONS}
\bigskip
\item{fig.1}: $\varepsilon, {\dot\varepsilon}, {\ddot\varepsilon}$ as
functions of $\tau$.  These are called gamma1, gamma2, and gamma3,
respectively, on the figures. To make the second and third figures convenient
 to represent, we have added  $150$ to the values of the
second, and $5 \times 10^3$ to the last, assuring positivity (and
value greater than unity) in our data range, and taken the logarithm
base 10. Recursive, approximate quasiperiodic behavior is clearly visible in
the variables $ {\dot\varepsilon}, {\ddot\varepsilon}$.
\smallskip
\item{fig.2}: The orbit as it enters the region of the attractor,
shown in the space of $ {\dot\varepsilon}, {\ddot\varepsilon}$,
showing the transition from the initial conditions to the strange
attractor.  In $\tau$, the curve starts on the ${\dot\varepsilon}$
axis to the right of the origin, and ends at the lower left of the origin.
\smallskip
\item{fig.3}: This curve continues the evolution within the
attractor, starting in the neighborhood of the origin, winding up and
around to the right and terminating almost at the same point (a little
above), coming in from the right.
\smallskip
\item{fig.4}:  This curve is a magnification the motion in the
neighborhood of the end point of figure 3, starting below the axis and
moving to the left.  It makes another loop, and ends in a smaller
pattern.
\smallskip
\item{fig.5}:  The smaller pattern approached in figure 4 is shown in
detail, now displaying a somewhat different general pattern.  Here, 
${\ddot\varepsilon}$ enters oscillations as $\varepsilon$ approaches
the neighborhood of unity.  Figures 5a and 5b show enlargements
of the innner loop, and figure 5c shows the endpoint in more detail.
\smallskip
\item{fig.6}:  $ {\dot\varepsilon}, \varepsilon$ plane in the $\tau$
interval represented in fig. 2.
\smallskip
\item{fig7a}: $ {\dot\varepsilon}, \varepsilon$ plane in the $\tau$  
interval represented in figure 3.
\smallskip
\item{fig.7b}:  $ {\dot\varepsilon}, \varepsilon$ plane in the $\tau$  
interval represented in figure 4, including the details corresponding
to figure 5.
\smallskip
\item{fig.8}: Largest averaged Lyapunov exponent (the values must be
divided by the size of the interval $10^{-7}$) as a function of the
accumulated $\tau$. We have used interval $0.4 \times 10^{-6}$.  Note
the sharp jump at approximately $10,400$ steps, indicating the
development of a very large instability in this neighborhood (the
additional terms here are divided by $10^4$, the number of time steps. 
\smallskip
\item{fig.9}: The time series for $\varepsilon(\tau)$ on a three
dimensional space corresponding to shift by 20 time steps.
\smallskip  
\item{fig.10}: The time series for ${\dot\varepsilon}(\tau)$ on a three
dimensional space corresponding to shift by 40 time steps.
\smallskip
\item{fig.11}: The time series for ${\ddot\varepsilon}(\tau)$ on a three
dimensional space corresponding to shift by 20 time steps.
\item{fig.12.}: In these figures, showing ${\dot \varepsilon}$
vs. $\varepsilon$  and ${\ddot \varepsilon}$ vs. ${\dot
\varepsilon}$, we have changed the initial conditions, and find a
similar pattern.

\vfill
\bye
\end














